Translate and Label! An Encoder-Decoder Approach for Cross-lingual Semantic Role Labeling

We propose a Cross-lingual Encoder-Decoder model that simultaneously translates and generates sentences with Semantic Role Labeling annotations in a resource-poor target language. Unlike annotation projection techniques, our model does not need parallel data during inference time. Our approach can be applied in monolingual, multilingual and cross-lingual settings and is able to produce dependency-based and span-based SRL annotations. We benchmark the labeling performance of our model in different monolingual and multilingual settings using well-known SRL datasets. We then train our model in a cross-lingual setting to generate new SRL labeled data. Finally, we measure the effectiveness of our method by using the generated data to augment the training basis for resource-poor languages and perform manual evaluation to show that it produces high-quality sentences and assigns accurate semantic role annotations. Our proposed architecture offers a flexible method for leveraging SRL data in multiple languages.

==> tables/CoNLL05.tex <==

\begin{table}[t!]
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{llll}
\hline
\multicolumn{4}{c}{English CoNLL-05 (Span Based)}                          \\ \hline
Model                                   & Dev   & WSJ Test & Brown Test \\  \hline
Zhou, 2016                       & 79.6  & 82.8     & 69.4       \\
He, 2017                         & 82.7  & 84.6     & 73.6       \\
Daza, 2018{[}S2S{]}               & 77.29 & 79.23    & 68.39      \\
Ours {[}S2S{]}                               & 82.3 & 81.8    & 72.7      \\ \hline
Strubell, 2018 {[}ELMo{]} & 85.4 & 86.9     & 78.3      \\
Ouchi, 2018 {[}ELMo{]}     & 87.4  & 88.5     & 79.6       \\
Ours + ELMo                        & 84.8     & 0        & 77.5          \\
Ours + BERT                        & 84.9  & 85.7    & 78.1     
\end{tabular}
}
\caption{F1 measure for argument role labeling of our seq2seq model w/ Attention \& Copying on CoNLL-05 dev and test sets compared to sequence labeling (Zhou \& Xu, He single model) and a previous S2S model. Bottom part shows models that use contextual representations; we compare to Strubell Syntax-Aware + ELMo model and Ouchi with ELMo model . \anette{[AF: Include newer models in top part (Strubell, He et al. 2018 (argument only)] \textcolor{red}{Do all of the benchmarking systems include nominal predicates; no separate evaluation? What did they do for the cyclic structures? Eliminated these roles? Can you adopt their solutions? }}
}
\label{SoA-2005}
\end{table}

==> tables/CoNLL09.tex <==

\begin{table}[t!]
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lllll}
\hline
\multicolumn{3}{c}{English CoNLL 2009 (Head-Based)}                                     \\ \hline
Model                                       & Test  & Test-OOD \\ \hline
FitzGerald, 2015              & 87.8  & 75.9 \\
Roth, 2016                                  & 87.7  & 76.1  \\
Marcheggiani, 2017                          & 89.1  & 78.9  \\
(Cai et al, 2018)                           & 89.6  & 79    \\
Ours {[}Mono{]}*                            & 82.9 & 75.3   \\ \hline
Li et al, 2019 {[}ELMo{]}                 & 90.4  & -     \\
Ours {[}Mono + BERT{]}*                     & 0     & 0 \\ \hline
\end{tabular}
}
\caption{F1 measure for argument role labeling on English CoNLL-09 head-based data. We compare our English monolingual model with the sequence labeling state-of-the-art models. Note that our models are only evaluated on verbal predicates.
}
\label{SoA-2009}
\end{table}

==> tables/DataMulti.tex <==
\begin{table}[t!]
\centering
\resizebox{0.43\textwidth}{!}{
\begin{tabular}{|llll|}
\hline
One-to-One Model            & EN     & DE     & FR     \\ \hline
\multicolumn{1}{|l|}{Train} & 88,260 & 37,177 & 69,446 \\
\multicolumn{1}{|l|}{Dev}   & 2,798  & 1,173  & 2,183  \\
\multicolumn{1}{|l|}{Test}   & 1,850  & 788  & 1,465  \\ \hline
\end{tabular}
}
\caption{Dataset split used for One-to-One Multilingual Models. \textit{EN} and \textit{DE} are taken from CoNLL-09 corpus; \textit{FR}: van der Plas 2011 (train \& dev), 2010 (test).}
\label{Data-Multi}
\end{table}

==> tables/HyperParam.tex <==
\begin{table}[t!]
\centering
\resizebox{0.5\textwidth}{!}{

\begin{tabular}{|ll|}
\hline
Parameter                                      & Size                 \\ \hline
Encoder Embedding Size {[}GloVe, BERT, ELMo{]} & {[}300, 768, 1024{]} \\
Vocabulary Size                                & Freq $>$ 5                  \\
Encoder Hidden                                 & 300                  \\
Decoder Hidden                                 & 300                  \\
Attention                                      & 1024                 \\
Language Embedding Size                        & 200                  \\
Predicate Indicator                            & 100                  \\
Epochs                                         & 30                   \\
Early Stopping Patience                        & 5 epochs             \\
Optimizer                                      & Adam                 \\
Learning Rate                                  & 0.0001               \\
Batch Size {[}GloVe, Other{]}                  & {[}32, 12{]}         \\
Gradient Clipping                              & 5                    \\
Dropout                                        & 0.1                  \\ \hline
\end{tabular}

}
\caption{Hyper-parameters used in our models}
\label{table:hyper}
\end{table}
